Pair-distribution function of active Brownian spheres in two spatial dimensions: simulation results and analytic representation

We investigate the full pair-distribution function of a homogeneous suspension of spherical active Brownian particles interacting by a Weeks-Chandler-Andersen potential in two spatial dimensions. The full pair-distribution function depends on three coordinates describing the relative positions and orientations of two particles, the P\'eclet number specifying the activity of the particles, and their mean packing density. This five-dimensional function is obtained from Brownian dynamics simulations. We discuss its structure taking into account all of its degrees of freedom. In addition, we present an approximate analytic expression for the product of the full pair-distribution function and the interparticle force. We find that the analytic expression, which is typically needed when deriving analytic models for the collective dynamics of active Brownian particles, is in good agreement with the simulation results. The results of this work can thus be expected to be helpful for the further theoretical investigation of active Brownian particles as well as nonequilibrium statistical physics in general.

==> fit_parameters_1.tex <==
\multicolumn{3}{c|}{}&$\uc_{-2,0}$&$\uc_{-1,0}$&$\uc_{0,0}$&$\uc_{1,0}$&$\uc_{2,0}$&$\uc_{-2,1}$&$\uc_{-1,1}$\\
\multicolumn{3}{c|}{}&$\uc_{0,1}$&$\uc_{1,1}$&$\uc_{2,1}$&$\uc_{-2,2}$&$\uc_{-1,2}$&$\uc_{0,2}$&$\uc_{1,2}$\\
\multicolumn{3}{c|}{}&$\uc_{2,2}$&$\uc_{-2,3}$ or $v$&$\uc_{-1,3}$ or $w$&$\uc_{0,3}$&$\uc_{1,3}$&$\uc_{2,3}$&\\
\hline
\multirow{12}{*}{$f^{11}_{00}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_{2,1}$} & $1.289\cdot 10^{6}$ & $4.177\cdot 10^{2}$ & $-1.155$ & $5.622$ & $-1.266\cdot 10^{-1}$ & $-3.875\cdot 10^{5}$ & $-2.458\cdot 10^{3}$\\
 &  &  & $4.829\cdot 10^{2}$ & $-3.689\cdot 10^{1}$ & $9.331\cdot 10^{-1}$ & $5.026\cdot 10^{4}$ & $2.266\cdot 10^{3}$ & $-3.870\cdot 10^{2}$ & $4.811\cdot 10^{1}$\\
 &  &  & $-1.439$ & $-1.289\cdot 10^{6}$ & $-3.050\cdot 10^{-1}$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $4.053\cdot 10^{-1}$ & $-6.079\cdot 10^{-1}$ & $1.094$ & $-5.760\cdot 10^{-3}$ & $1.276\cdot 10^{-4}$ & $-7.771\cdot 10^{-1}$ & $6.193\cdot 10^{-1}$\\
 &  &  & $-1.317\cdot 10^{-1}$ & $7.476\cdot 10^{-3}$ & $-1.486\cdot 10^{-4}$ & $-1.011$ & $7.427\cdot 10^{-1}$ & $-2.279\cdot 10^{-1}$ & $1.772\cdot 10^{-2}$\\
 &  &  & $-5.755\cdot 10^{-4}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $-6.346\cdot 10^{-2}$ & $5.995\cdot 10^{-2}$ & $2.773\cdot 10^{-2}$ & $-1.531\cdot 10^{-3}$ & $2.978\cdot 10^{-5}$ & $1.252\cdot 10^{-1}$ & $-1.030\cdot 10^{-1}$\\
 &  &  & $3.087\cdot 10^{-2}$ & $-3.739\cdot 10^{-3}$ & $1.647\cdot 10^{-4}$ & $-1.189$ & $9.590\cdot 10^{-1}$ & $-2.733\cdot 10^{-1}$ & $2.890\cdot 10^{-2}$\\
 &  &  & $-8.597\cdot 10^{-4}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $1.992\cdot 10^{2}$ & $-1.300\cdot 10^{2}$ & $3.012\cdot 10^{1}$ & $-3.009\cdot 10^{-1}$ & $-1.116\cdot 10^{-2}$ & $-2.011\cdot 10^{1}$ & $-1.553\cdot 10^{1}$\\
 &  &  & $1.583\cdot 10^{1}$ & $-2.333$ & $1.240\cdot 10^{-1}$ & $-5.742\cdot 10^{2}$ & $4.400\cdot 10^{2}$ & $-1.159\cdot 10^{2}$ & $1.343\cdot 10^{1}$\\
 &  &  & $-4.194\cdot 10^{-1}$ & $3.578\cdot 10^{-4}$ & $1.068\cdot 10^{1}$ &  &  &  & 
\\ \hline
\multirow{15}{*}{$f^{11}_{01}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_3$} & $-1.356\cdot 10^{5}$ & $9.625\cdot 10^{4}$ & $-1.791\cdot 10^{4}$ & $1.447\cdot 10^{3}$ & $-3.832\cdot 10^{1}$ & $7.551\cdot 10^{5}$ & $-5.194\cdot 10^{5}$\\
 &  &  & $1.026\cdot 10^{5}$ & $-7.796\cdot 10^{3}$ & $1.981\cdot 10^{2}$ & $-1.297\cdot 10^{6}$ & $8.589\cdot 10^{5}$ & $-1.672\cdot 10^{5}$ & $1.151\cdot 10^{4}$\\
 &  &  & $-2.391\cdot 10^{2}$ & $4.751\cdot 10^{5}$ & $-2.628\cdot 10^{5}$ & $2.960\cdot 10^{4}$ & $1.845\cdot 10^{3}$ & $-2.210\cdot 10^{2}$ & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $3.877\cdot 10^{-1}$ & $-5.949\cdot 10^{-1}$ & $1.085$ & $-4.761\cdot 10^{-3}$ & $9.649\cdot 10^{-5}$ & $-1.667\cdot 10^{-1}$ & $2.675\cdot 10^{-1}$\\
 &  &  & $-7.688\cdot 10^{-2}$ & $3.997\cdot 10^{-3}$ & $-7.668\cdot 10^{-5}$ & $-1.862$ & $1.233$ & $-3.051\cdot 10^{-1}$ & $2.196\cdot 10^{-2}$\\
 &  &  & $-5.631\cdot 10^{-4}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $-7.823\cdot 10^{-2}$ & $6.839\cdot 10^{-2}$ & $2.250\cdot 10^{-2}$ & $-1.057\cdot 10^{-3}$ & $1.629\cdot 10^{-5}$ & $3.272\cdot 10^{-1}$ & $-2.324\cdot 10^{-1}$\\
 &  &  & $5.708\cdot 10^{-2}$ & $-5.948\cdot 10^{-3}$ & $2.247\cdot 10^{-4}$ & $-1.461$ & $1.135$ & $-3.085\cdot 10^{-1}$ & $3.173\cdot 10^{-2}$\\
 &  &  & $-9.244\cdot 10^{-4}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $2.708\cdot 10^{1}$ & $3.225\cdot 10^{1}$ & $-2.651\cdot 10^{1}$ & $4.929$ & $-1.413\cdot 10^{-1}$ & $1.114\cdot 10^{2}$ & $-1.483\cdot 10^{2}$\\
 &  &  & $5.656\cdot 10^{1}$ & $-6.330$ & $2.456\cdot 10^{-1}$ & $-4.180\cdot 10^{2}$ & $2.683\cdot 10^{2}$ & $-4.662\cdot 10^{1}$ & $2.048$\\
 &  &  & $3.428\cdot 10^{-1}$ & $1.179\cdot 10^{-2}$ & $7.430$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$r_1$} & \multirow{3}{*}{$h_3$} & $-4.383\cdot 10^{-1}$ & $3.225\cdot 10^{-1}$ & $1.063$ & $3.207\cdot 10^{-3}$ & $-9.131\cdot 10^{-5}$ & $6.826$ & $-5.178$\\
 &  &  & $1.210$ & $-1.216\cdot 10^{-1}$ & $4.080\cdot 10^{-3}$ & $-3.504\cdot 10^{1}$ & $2.632\cdot 10^{1}$ & $-6.334$ & $6.274\cdot 10^{-1}$\\
 &  &  & $-2.149\cdot 10^{-2}$ & $4.976\cdot 10^{1}$ & $-3.827\cdot 10^{1}$ & $9.697$ & $-1.049$ & $3.833\cdot 10^{-2}$ & 
\\ \hline
\multirow{15}{*}{$f^{11}_{02}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_3$} & $5.620\cdot 10^{3}$ & $-4.484\cdot 10^{3}$ & $1.327\cdot 10^{3}$ & $-1.855\cdot 10^{2}$ & $2.450$ & $-1.411\cdot 10^{4}$ & $1.228\cdot 10^{4}$\\
 &  &  & $-3.597\cdot 10^{3}$ & $3.792\cdot 10^{2}$ & $-3.297$ & $3.206\cdot 10^{4}$ & $-2.887\cdot 10^{4}$ & $8.517\cdot 10^{3}$ & $-8.569\cdot 10^{2}$\\
 &  &  & $1.980\cdot 10^{1}$ & $-5.706\cdot 10^{4}$ & $4.674\cdot 10^{4}$ & $-1.279\cdot 10^{4}$ & $1.243\cdot 10^{3}$ & $-3.226\cdot 10^{1}$ & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $5.440\cdot 10^{-1}$ & $-6.862\cdot 10^{-1}$ & $1.094$ & $-4.350\cdot 10^{-3}$ & $7.520\cdot 10^{-5}$ & $-6.827\cdot 10^{-1}$ & $4.410\cdot 10^{-1}$\\
 &  &  & $-5.747\cdot 10^{-2}$ & $-3.190\cdot 10^{-3}$ & $2.566\cdot 10^{-4}$ & $-3.161$ & $2.514$ & $-7.143\cdot 10^{-1}$ & $7.068\cdot 10^{-2}$\\
 &  &  & $-2.286\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $-4.278\cdot 10^{-2}$ & $4.922\cdot 10^{-2}$ & $2.434\cdot 10^{-2}$ & $-1.018\cdot 10^{-3}$ & $1.465\cdot 10^{-5}$ & $1.647\cdot 10^{-1}$ & $-1.737\cdot 10^{-1}$\\
 &  &  & $5.786\cdot 10^{-2}$ & $-7.240\cdot 10^{-3}$ & $2.832\cdot 10^{-4}$ & $-1.515$ & $1.266$ & $-3.628\cdot 10^{-1}$ & $3.930\cdot 10^{-2}$\\
 &  &  & $-1.238\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $-6.112\cdot 10^{1}$ & $9.041\cdot 10^{1}$ & $9.555\cdot 10^{3}$ & $9.617$ & $-2.635\cdot 10^{-1}$ & $1.354\cdot 10^{2}$ & $-1.977\cdot 10^{2}$\\
 &  &  & $-3.869\cdot 10^{3}$ & $-2.213\cdot 10^{1}$ & $8.787\cdot 10^{-1}$ & $-3.251\cdot 10^{3}$ & $2.567\cdot 10^{3}$ & $-7.010$ & $8.860\cdot 10^{1}$\\
 &  &  & $-2.958$ & $-9.600\cdot 10^{3}$ & $-4.187\cdot 10^{-1}$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$r_1$} & \multirow{3}{*}{$h_3$} & $-3.578\cdot 10^{-1}$ & $2.130\cdot 10^{-1}$ & $9.909\cdot 10^{-1}$ & $2.343\cdot 10^{-3}$ & $-6.252\cdot 10^{-5}$ & $7.756\cdot 10^{-1}$ & $-5.331\cdot 10^{-1}$\\
 &  &  & $1.441\cdot 10^{-1}$ & $-1.304\cdot 10^{-2}$ & $3.845\cdot 10^{-4}$ & $-3.366$ & $1.084$ & $-2.252\cdot 10^{-1}$ & $1.073\cdot 10^{-2}$\\
 &  &  & $-3.055\cdot 10^{-4}$ & $2.248\cdot 10^{-1}$ & $1.190$ & $-5.167\cdot 10^{-1}$ & $5.657\cdot 10^{-2}$ & $-1.533\cdot 10^{-3}$ & 
\\ \hline


==> fit_parameters_2.tex <==
\multicolumn{3}{c|}{}&$\uc_{-2,0}$&$\uc_{-1,0}$&$\uc_{0,0}$&$\uc_{1,0}$&$\uc_{2,0}$&$\uc_{-2,1}$&$\uc_{-1,1}$\\
\multicolumn{3}{c|}{}&$\uc_{0,1}$&$\uc_{1,1}$&$\uc_{2,1}$&$\uc_{-2,2}$&$\uc_{-1,2}$&$\uc_{0,2}$&$\uc_{1,2}$\\
\multicolumn{3}{c|}{}&$\uc_{2,2}$&$\uc_{-2,3}$ or $v$&$\uc_{-1,3}$ or $w$&$\uc_{0,3}$&$\uc_{1,3}$&$\uc_{2,3}$&\\
\hline
\multirow{15}{*}{$f^{11}_{10}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_3$} & $3.641\cdot 10^{4}$ & $-2.547\cdot 10^{4}$ & $4.944\cdot 10^{3}$ & $-4.551\cdot 10^{2}$ & $1.012\cdot 10^{1}$ & $-1.992\cdot 10^{5}$ & $1.297\cdot 10^{5}$\\
 &  &  & $-2.211\cdot 10^{4}$ & $1.373\cdot 10^{3}$ & $-2.151\cdot 10^{1}$ & $3.206\cdot 10^{5}$ & $-1.868\cdot 10^{5}$ & $2.375\cdot 10^{4}$ & $-2.328\cdot 10^{2}$\\
 &  &  & $-7.111\cdot 10^{1}$ & $-2.240\cdot 10^{4}$ & $-3.194\cdot 10^{4}$ & $2.807\cdot 10^{4}$ & $-5.088\cdot 10^{3}$ & $2.681\cdot 10^{2}$ & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $5.170\cdot 10^{-1}$ & $-6.399\cdot 10^{-1}$ & $1.081$ & $-3.472\cdot 10^{-3}$ & $4.618\cdot 10^{-5}$ & $-7.545\cdot 10^{-1}$ & $3.477\cdot 10^{-1}$\\
 &  &  & $-2.897\cdot 10^{-2}$ & $-4.733\cdot 10^{-3}$ & $2.706\cdot 10^{-4}$ & $-2.845$ & $2.402$ & $-6.798\cdot 10^{-1}$ & $6.604\cdot 10^{-2}$\\
 &  &  & $-2.033\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $-9.639\cdot 10^{-2}$ & $8.708\cdot 10^{-2}$ & $1.608\cdot 10^{-2}$ & $-3.764\cdot 10^{-4}$ & $-4.711\cdot 10^{-6}$ & $3.567\cdot 10^{-1}$ & $-3.154\cdot 10^{-1}$\\
 &  &  & $8.479\cdot 10^{-2}$ & $-8.871\cdot 10^{-3}$ & $3.170\cdot 10^{-4}$ & $-1.575$ & $1.300$ & $-3.551\cdot 10^{-1}$ & $3.704\cdot 10^{-2}$\\
 &  &  & $-1.104\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $1.568\cdot 10^{2}$ & $-2.905\cdot 10^{1}$ & $-2.501\cdot 10^{1}$ & $6.921$ & $-2.253\cdot 10^{-1}$ & $4.375\cdot 10^{2}$ & $-5.432\cdot 10^{2}$\\
 &  &  & $2.087\cdot 10^{2}$ & $-2.526\cdot 10^{1}$ & $9.676\cdot 10^{-1}$ & $-3.219\cdot 10^{3}$ & $2.582\cdot 10^{3}$ & $-7.048\cdot 10^{2}$ & $8.090\cdot 10^{1}$\\
 &  &  & $-2.749$ & $1.250\cdot 10^{-10}$ & $2.821\cdot 10^{1}$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$r_1$} & \multirow{3}{*}{$h_3$} & $-1.286$ & $5.267\cdot 10^{-1}$ & $1.083$ & $-7.543\cdot 10^{-3}$ & $2.611\cdot 10^{-4}$ & $5.947$ & $-1.231$\\
 &  &  & $1.026\cdot 10^{-1}$ & $-6.934\cdot 10^{-3}$ & $3.060\cdot 10^{-4}$ & $-1.907\cdot 10^{1}$ & $8.525$ & $-2.872$ & $2.511\cdot 10^{-1}$\\
 &  &  & $-8.224\cdot 10^{-3}$ & $1.748\cdot 10^{1}$ & $-1.081\cdot 10^{1}$ & $3.520$ & $-3.424\cdot 10^{-1}$ & $1.213\cdot 10^{-2}$ & 
\\ \hline
\multirow{15}{*}{$f^{11}_{11}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_3$} & $-3.196\cdot 10^{4}$ & $2.868\cdot 10^{4}$ & $-5.314\cdot 10^{3}$ & $4.779\cdot 10^{2}$ & $-1.077\cdot 10^{1}$ & $1.027\cdot 10^{5}$ & $-9.872\cdot 10^{4}$\\
 &  &  & $2.203\cdot 10^{4}$ & $-1.613\cdot 10^{3}$ & $2.998\cdot 10^{1}$ & $-9.436\cdot 10^{4}$ & $9.754\cdot 10^{4}$ & $-2.223\cdot 10^{4}$ & $6.200\cdot 10^{2}$\\
 &  &  & $4.210\cdot 10^{1}$ & $-1.409\cdot 10^{5}$ & $1.079\cdot 10^{5}$ & $-3.457\cdot 10^{4}$ & $5.841\cdot 10^{3}$ & $-2.912\cdot 10^{2}$ & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $3.534\cdot 10^{-1}$ & $-5.574\cdot 10^{-1}$ & $1.072$ & $-3.666\cdot 10^{-3}$ & $7.260\cdot 10^{-5}$ & $-1.773\cdot 10^{-1}$ & $2.565\cdot 10^{-1}$\\
 &  &  & $-6.534\cdot 10^{-2}$ & $2.536\cdot 10^{-3}$ & $-4.109\cdot 10^{-5}$ & $-1.884$ & $1.251$ & $-3.110\cdot 10^{-1}$ & $2.203\cdot 10^{-2}$\\
 &  &  & $-4.862\cdot 10^{-4}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $-4.619\cdot 10^{-2}$ & $5.229\cdot 10^{-2}$ & $2.474\cdot 10^{-2}$ & $-1.276\cdot 10^{-3}$ & $2.427\cdot 10^{-5}$ & $1.326\cdot 10^{-1}$ & $-1.182\cdot 10^{-1}$\\
 &  &  & $3.585\cdot 10^{-2}$ & $-4.237\cdot 10^{-3}$ & $1.699\cdot 10^{-4}$ & $-1.195$ & $9.595\cdot 10^{-1}$ & $-2.689\cdot 10^{-1}$ & $2.794\cdot 10^{-2}$\\
 &  &  & $-7.915\cdot 10^{-4}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $-1.030\cdot 10^{2}$ & $1.461\cdot 10^{2}$ & $-6.233\cdot 10^{1}$ & $9.356$ & $-2.241\cdot 10^{-1}$ & $2.393\cdot 10^{2}$ & $-2.989\cdot 10^{2}$\\
 &  &  & $1.146\cdot 10^{2}$ & $-1.355\cdot 10^{1}$ & $3.712\cdot 10^{-1}$ & $4.241\cdot 10^{2}$ & $-4.257\cdot 10^{2}$ & $1.623\cdot 10^{2}$ & $-2.811\cdot 10^{1}$\\
 &  &  & $2.009$ & $3.352\cdot 10^{-2}$ & $6.497$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$r_1$} & \multirow{3}{*}{$h_3$} & $2.555\cdot 10^{-1}$ & $-1.456\cdot 10^{-1}$ & $1.182$ & $-1.057\cdot 10^{-2}$ & $2.431\cdot 10^{-4}$ & $1.614\cdot 10^{-1}$ & $-4.457\cdot 10^{-1}$\\
 &  &  & $-1.808\cdot 10^{-2}$ & $7.986\cdot 10^{-3}$ & $-1.921\cdot 10^{-5}$ & $-7.272$ & $5.457$ & $-7.552\cdot 10^{-1}$ & $3.301\cdot 10^{-2}$\\
 &  &  & $-1.667\cdot 10^{-3}$ & $6.677$ & $-4.969$ & $6.517\cdot 10^{-1}$ & $-6.629\cdot 10^{-2}$ & $4.739\cdot 10^{-3}$ & 
\\ \hline
\multirow{18}{*}{$f^{11}_{12}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_3$} & $-4.364\cdot 10^{4}$ & $9.766\cdot 10^{3}$ & $5.877\cdot 10^{3}$ & $-1.853\cdot 10^{3}$ & $-1.252\cdot 10^{1}$ & $4.023\cdot 10^{6}$ & $-3.048\cdot 10^{6}$\\
 &  &  & $8.156\cdot 10^{5}$ & $-9.070\cdot 10^{4}$ & $3.420\cdot 10^{3}$ & $-1.991\cdot 10^{7}$ & $1.563\cdot 10^{7}$ & $-4.337\cdot 10^{6}$ & $4.974\cdot 10^{5}$\\
 &  &  & $-1.902\cdot 10^{4}$ & $3.745\cdot 10^{7}$ & $-3.017\cdot 10^{7}$ & $8.634\cdot 10^{6}$ & $-1.029\cdot 10^{6}$ & $4.198\cdot 10^{4}$ & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $1.390$ & $-1.370$ & $1.264$ & $-2.252\cdot 10^{-2}$ & $6.813\cdot 10^{-4}$ & $-2.623$ & $2.207$\\
 &  &  & $-5.610\cdot 10^{-1}$ & $5.258\cdot 10^{-2}$ & $-1.710\cdot 10^{-3}$ & $-1.429\cdot 10^{-1}$ & $-2.820\cdot 10^{-1}$ & $1.256\cdot 10^{-1}$ & $-3.004\cdot 10^{-2}$\\
 &  &  & $1.735\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $-8.053\cdot 10^{-3}$ & $1.404\cdot 10^{-2}$ & $4.011\cdot 10^{-2}$ & $-2.327\cdot 10^{-3}$ & $3.380\cdot 10^{-5}$ & $7.970\cdot 10^{-2}$ & $3.213\cdot 10^{-3}$\\
 &  &  & $1.666\cdot 10^{-3}$ & $-4.446\cdot 10^{-4}$ & $6.597\cdot 10^{-5}$ & $-5.394\cdot 10^{-1}$ & $4.124\cdot 10^{-1}$ & $-1.209\cdot 10^{-1}$ & $1.210\cdot 10^{-2}$\\
 &  &  & $-3.351\cdot 10^{-4}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $-1.228\cdot 10^{3}$ & $8.470\cdot 10^{2}$ & $-1.994\cdot 10^{2}$ & $2.383\cdot 10^{1}$ & $-7.986\cdot 10^{-1}$ & $3.551\cdot 10^{3}$ & $-2.227\cdot 10^{3}$\\
 &  &  & $5.049\cdot 10^{2}$ & $-4.983\cdot 10^{1}$ & $1.891$ & $-3.867\cdot 10^{3}$ & $2.612\cdot 10^{3}$ & $-6.786\cdot 10^{2}$ & $8.736\cdot 10^{1}$\\
 &  &  & $-4.084$ & $3.253\cdot 10^{-7}$ & $2.033\cdot 10^{1}$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$r_1$} & \multirow{3}{*}{$h_3$} & $1.187$ & $-9.285\cdot 10^{-1}$ & $9.999\cdot 10^{-1}$ & $3.763\cdot 10^{-3}$ & $-2.319\cdot 10^{-4}$ & $-2.820\cdot 10^{1}$ & $1.856\cdot 10^{1}$\\
 &  &  & $-4.263$ & $4.173\cdot 10^{-1}$ & $-1.482\cdot 10^{-2}$ & $8.351\cdot 10^{1}$ & $-5.845\cdot 10^{1}$ & $1.462\cdot 10^{1}$ & $-1.588$\\
 &  &  & $6.166\cdot 10^{-2}$ & $-1.183\cdot 10^{2}$ & $9.199\cdot 10^{1}$ & $-2.595\cdot 10^{1}$ & $3.163$ & $-1.390\cdot 10^{-1}$ & \\
\cline{3-10} & \multirow{3}{*}{$r_2$} & \multirow{3}{*}{$h_3$} & $-9.328\cdot 10^{-2}$ & $-2.678\cdot 10^{-2}$ & $1.037$ & $9.548\cdot 10^{-4}$ & $-6.395\cdot 10^{-5}$ & $4.177$ & $-3.739$\\
 &  &  & $8.652\cdot 10^{-1}$ & $-8.863\cdot 10^{-2}$ & $2.853\cdot 10^{-3}$ & $-2.336\cdot 10^{1}$ & $1.746\cdot 10^{1}$ & $-4.658$ & $4.671\cdot 10^{-1}$\\
 &  &  & $-1.513\cdot 10^{-2}$ & $2.890\cdot 10^{1}$ & $-2.176\cdot 10^{1}$ & $5.886$ & $-6.174\cdot 10^{-1}$ & $2.042\cdot 10^{-2}$ & 
\\ \hline


==> fit_parameters_3.tex <==
\multicolumn{3}{c|}{}&$\uc_{-2,0}$&$\uc_{-1,0}$&$\uc_{0,0}$&$\uc_{1,0}$&$\uc_{2,0}$&$\uc_{-2,1}$&$\uc_{-1,1}$\\
\multicolumn{3}{c|}{}&$\uc_{0,1}$&$\uc_{1,1}$&$\uc_{2,1}$&$\uc_{-2,2}$&$\uc_{-1,2}$&$\uc_{0,2}$&$\uc_{1,2}$\\
\multicolumn{3}{c|}{}&$\uc_{2,2}$&$\uc_{-2,3}$ or $v$&$\uc_{-1,3}$ or $w$&$\uc_{0,3}$&$\uc_{1,3}$&$\uc_{2,3}$&\\
\hline
\multirow{18}{*}{$f^{11}_{20}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_3$} & $3.262\cdot 10^{4}$ & $-1.514\cdot 10^{4}$ & $1.535\cdot 10^{3}$ & $-2.931\cdot 10^{1}$ & $6.543\cdot 10^{1}$ & $-9.851\cdot 10^{5}$ & $6.975\cdot 10^{5}$\\
 &  &  & $-1.719\cdot 10^{5}$ & $1.717\cdot 10^{4}$ & $-7.445\cdot 10^{2}$ & $3.652\cdot 10^{6}$ & $-2.717\cdot 10^{6}$ & $7.044\cdot 10^{5}$ & $-7.338\cdot 10^{4}$\\
 &  &  & $2.652\cdot 10^{3}$ & $-3.786\cdot 10^{6}$ & $2.906\cdot 10^{6}$ & $-7.814\cdot 10^{5}$ & $8.528\cdot 10^{4}$ & $-3.128\cdot 10^{3}$ & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $3.916\cdot 10^{-1}$ & $-5.494\cdot 10^{-1}$ & $1.070$ & $-2.369\cdot 10^{-3}$ & $1.913\cdot 10^{-5}$ & $1.434$ & $-1.359$\\
 &  &  & $3.691\cdot 10^{-1}$ & $-3.954\cdot 10^{-2}$ & $1.283\cdot 10^{-3}$ & $-6.296$ & $5.491$ & $-1.532$ & $1.524\cdot 10^{-1}$\\
 &  &  & $-4.754\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $-6.051\cdot 10^{-2}$ & $6.333\cdot 10^{-2}$ & $2.254\cdot 10^{-2}$ & $-8.503\cdot 10^{-4}$ & $6.868\cdot 10^{-6}$ & $3.272\cdot 10^{-1}$ & $-2.414\cdot 10^{-1}$\\
 &  &  & $8.596\cdot 10^{-2}$ & $-1.110\cdot 10^{-2}$ & $4.453\cdot 10^{-4}$ & $-2.731$ & $1.923$ & $-5.165\cdot 10^{-1}$ & $5.701\cdot 10^{-2}$\\
 &  &  & $-1.967\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $7.071\cdot 10^{1}$ & $9.245\cdot 10^{1}$ & $1.621\cdot 10^{4}$ & $9.781$ & $-2.805\cdot 10^{-1}$ & $-8.229\cdot 10^{2}$ & $-2.028\cdot 10^{2}$\\
 &  &  & $-4.783\cdot 10^{3}$ & $-3.426\cdot 10^{1}$ & $1.321$ & $-2.758\cdot 10^{3}$ & $3.198\cdot 10^{3}$ & $-3.568\cdot 10^{2}$ & $1.344\cdot 10^{2}$\\
 &  &  & $-4.789$ & $-1.627\cdot 10^{4}$ & $-3.091\cdot 10^{-1}$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$r_1$} & \multirow{3}{*}{$h_3$} & $1.646$ & $-1.436$ & $1.215$ & $-1.231\cdot 10^{-2}$ & $2.812\cdot 10^{-4}$ & $-1.002$ & $-8.863\cdot 10^{-1}$\\
 &  &  & $3.140\cdot 10^{-1}$ & $-2.946\cdot 10^{-2}$ & $7.815\cdot 10^{-4}$ & $-1.755\cdot 10^{1}$ & $1.684\cdot 10^{1}$ & $-4.548$ & $3.860\cdot 10^{-1}$\\
 &  &  & $-1.063\cdot 10^{-2}$ & $3.746\cdot 10^{1}$ & $-3.044\cdot 10^{1}$ & $8.080$ & $-7.767\cdot 10^{-1}$ & $2.333\cdot 10^{-2}$ & \\
\cline{3-10} & \multirow{3}{*}{$r_2$} & \multirow{3}{*}{$h_3$} & $9.059\cdot 10^{-1}$ & $-1.829\cdot 10^{-1}$ & $1.089$ & $6.387\cdot 10^{-3}$ & $-3.854\cdot 10^{-4}$ & $2.458\cdot 10^{-1}$ & $-3.356$\\
 &  &  & $2.174$ & $-2.950\cdot 10^{-1}$ & $1.108\cdot 10^{-2}$ & $-4.929\cdot 10^{1}$ & $4.286\cdot 10^{1}$ & $-1.490\cdot 10^{1}$ & $1.679$\\
 &  &  & $-5.832\cdot 10^{-2}$ & $8.621\cdot 10^{1}$ & $-6.924\cdot 10^{1}$ & $2.070\cdot 10^{1}$ & $-2.267$ & $7.687\cdot 10^{-2}$ & 
\\ \hline
\multirow{18}{*}{$f^{11}_{21}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_3$} & $5.557\cdot 10^{4}$ & $-7.079\cdot 10^{4}$ & $1.715\cdot 10^{4}$ & $-1.715\cdot 10^{3}$ & $-1.776\cdot 10^{1}$ & $-2.156\cdot 10^{5}$ & $2.825\cdot 10^{5}$\\
 &  &  & $-4.954\cdot 10^{4}$ & $1.933\cdot 10^{3}$ & $1.669\cdot 10^{2}$ & $1.368\cdot 10^{6}$ & $-1.245\cdot 10^{6}$ & $2.867\cdot 10^{5}$ & $-2.528\cdot 10^{4}$\\
 &  &  & $7.764\cdot 10^{2}$ & $-4.187\cdot 10^{6}$ & $3.394\cdot 10^{6}$ & $-9.074\cdot 10^{5}$ & $9.857\cdot 10^{4}$ & $-3.665\cdot 10^{3}$ & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $1.882\cdot 10^{-1}$ & $-5.259\cdot 10^{-1}$ & $1.071$ & $-3.171\cdot 10^{-3}$ & $5.404\cdot 10^{-5}$ & $7.733\cdot 10^{-1}$ & $-2.626\cdot 10^{-1}$\\
 &  &  & $7.348\cdot 10^{-2}$ & $-1.274\cdot 10^{-2}$ & $5.236\cdot 10^{-4}$ & $-6.660$ & $4.802$ & $-1.270$ & $1.270\cdot 10^{-1}$\\
 &  &  & $-4.146\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $1.060\cdot 10^{-1}$ & $-5.702\cdot 10^{-2}$ & $4.575\cdot 10^{-2}$ & $-2.804\cdot 10^{-3}$ & $6.314\cdot 10^{-5}$ & $-6.956\cdot 10^{-1}$ & $3.783\cdot 10^{-1}$\\
 &  &  & $-4.457\cdot 10^{-2}$ & $2.390\cdot 10^{-4}$ & $1.079\cdot 10^{-4}$ & $-1.410$ & $1.272$ & $-3.958\cdot 10^{-1}$ & $4.609\cdot 10^{-2}$\\
 &  &  & $-1.596\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $-1.055\cdot 10^{1}$ & $5.062\cdot 10^{1}$ & $-3.404\cdot 10^{1}$ & $6.395$ & $-1.120\cdot 10^{-1}$ & $-6.162\cdot 10^{2}$ & $3.137\cdot 10^{2}$\\
 &  &  & $-1.303\cdot 10^{1}$ & $-6.257$ & $2.865\cdot 10^{-1}$ & $-2.943\cdot 10^{3}$ & $2.366\cdot 10^{3}$ & $-6.650\cdot 10^{2}$ & $8.050\cdot 10^{1}$\\
 &  &  & $-2.547$ & $2.233\cdot 10^{-5}$ & $1.410\cdot 10^{1}$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$r_1$} & \multirow{3}{*}{$h_3$} & $1.038$ & $-5.679\cdot 10^{-1}$ & $1.068$ & $-1.243\cdot 10^{-3}$ & $-2.006\cdot 10^{-5}$ & $2.342\cdot 10^{-1}$ & $-1.817$\\
 &  &  & $8.069\cdot 10^{-1}$ & $-9.209\cdot 10^{-2}$ & $3.094\cdot 10^{-3}$ & $-2.032\cdot 10^{1}$ & $1.695\cdot 10^{1}$ & $-5.364$ & $5.308\cdot 10^{-1}$\\
 &  &  & $-1.653\cdot 10^{-2}$ & $2.109\cdot 10^{1}$ & $-1.655\cdot 10^{1}$ & $4.900$ & $-4.785\cdot 10^{-1}$ & $1.384\cdot 10^{-2}$ & \\
\cline{3-10} & \multirow{3}{*}{$r_2$} & \multirow{3}{*}{$h_3$} & $7.914\cdot 10^{-1}$ & $-4.777\cdot 10^{-1}$ & $1.240$ & $-1.206\cdot 10^{-2}$ & $2.997\cdot 10^{-4}$ & $-1.221\cdot 10^{1}$ & $7.468$\\
 &  &  & $-1.483$ & $1.256\cdot 10^{-1}$ & $-3.795\cdot 10^{-3}$ & $3.867\cdot 10^{1}$ & $-2.554\cdot 10^{1}$ & $6.103$ & $-6.520\cdot 10^{-1}$\\
 &  &  & $2.428\cdot 10^{-2}$ & $-6.761\cdot 10^{1}$ & $5.032\cdot 10^{1}$ & $-1.388\cdot 10^{1}$ & $1.574$ & $-6.056\cdot 10^{-2}$ & 
\\ \hline
\multirow{15}{*}{$f^{11}_{22}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_3$} & $3.181\cdot 10^{3}$ & $-2.943\cdot 10^{3}$ & $1.034\cdot 10^{3}$ & $-1.738\cdot 10^{2}$ & $3.794$ & $-4.607\cdot 10^{1}$ & $3.692\cdot 10^{3}$\\
 &  &  & $-2.022\cdot 10^{3}$ & $3.100\cdot 10^{2}$ & $-8.373$ & $-7.021\cdot 10^{3}$ & $-3.370\cdot 10^{3}$ & $3.125\cdot 10^{3}$ & $-4.570\cdot 10^{2}$\\
 &  &  & $1.735\cdot 10^{1}$ & $-6.421\cdot 10^{2}$ & $6.042\cdot 10^{3}$ & $-2.792\cdot 10^{3}$ & $2.879\cdot 10^{2}$ & $-7.221$ & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $7.632\cdot 10^{-1}$ & $-8.366\cdot 10^{-1}$ & $1.128$ & $-7.494\cdot 10^{-3}$ & $1.431\cdot 10^{-4}$ & $-1.768$ & $1.144$\\
 &  &  & $-2.050\cdot 10^{-1}$ & $8.687\cdot 10^{-3}$ & $2.973\cdot 10^{-6}$ & $-2.322$ & $2.034$ & $-6.374\cdot 10^{-1}$ & $6.786\cdot 10^{-2}$\\
 &  &  & $-2.387\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $3.643\cdot 10^{-2}$ & $-3.122\cdot 10^{-3}$ & $3.526\cdot 10^{-2}$ & $-1.849\cdot 10^{-3}$ & $2.906\cdot 10^{-5}$ & $-2.354\cdot 10^{-1}$ & $8.167\cdot 10^{-2}$\\
 &  &  & $7.198\cdot 10^{-3}$ & $-3.667\cdot 10^{-3}$ & $2.186\cdot 10^{-4}$ & $-1.207$ & $1.091$ & $-3.367\cdot 10^{-1}$ & $3.876\cdot 10^{-2}$\\
 &  &  & $-1.290\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $4.978\cdot 10^{2}$ & $-2.921\cdot 10^{2}$ & $1.700\cdot 10^{4}$ & $1.886$ & $-1.017\cdot 10^{-1}$ & $-2.462\cdot 10^{3}$ & $1.585\cdot 10^{3}$\\
 &  &  & $-6.078\cdot 10^{3}$ & $1.469\cdot 10^{1}$ & $-6.208\cdot 10^{-2}$ & $-9.783\cdot 10^{1}$ & $3.717\cdot 10^{2}$ & $6.634\cdot 10^{2}$ & $4.290\cdot 10^{1}$\\
 &  &  & $-1.855$ & $-1.696\cdot 10^{4}$ & $-3.431\cdot 10^{-1}$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$r_1$} & \multirow{3}{*}{$h_3$} & $-4.263\cdot 10^{-1}$ & $2.202\cdot 10^{-1}$ & $9.980\cdot 10^{-1}$ & $1.907\cdot 10^{-3}$ & $-5.164\cdot 10^{-5}$ & $1.817$ & $-1.112$\\
 &  &  & $2.470\cdot 10^{-1}$ & $-2.305\cdot 10^{-2}$ & $6.989\cdot 10^{-4}$ & $-8.017$ & $4.376$ & $-1.034$ & $9.458\cdot 10^{-2}$\\
 &  &  & $-3.066\cdot 10^{-3}$ & $8.023$ & $-4.755$ & $1.059$ & $-1.122\cdot 10^{-1}$ & $4.125\cdot 10^{-3}$ & 
\\ \hline


==> fit_parameters_4.tex <==
\multicolumn{3}{c|}{}&$\uc_{-2,0}$&$\uc_{-1,0}$&$\uc_{0,0}$&$\uc_{1,0}$&$\uc_{2,0}$&$\uc_{-2,1}$&$\uc_{-1,1}$\\
\multicolumn{3}{c|}{}&$\uc_{0,1}$&$\uc_{1,1}$&$\uc_{2,1}$&$\uc_{-2,2}$&$\uc_{-1,2}$&$\uc_{0,2}$&$\uc_{1,2}$\\
\multicolumn{3}{c|}{}&$\uc_{2,2}$&$\uc_{-2,3}$ or $v$&$\uc_{-1,3}$ or $w$&$\uc_{0,3}$&$\uc_{1,3}$&$\uc_{2,3}$&\\
\hline
\multirow{15}{*}{$f^{22}_{11}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_3$} & $-3.196\cdot 10^{4}$ & $2.868\cdot 10^{4}$ & $-5.314\cdot 10^{3}$ & $4.779\cdot 10^{2}$ & $-1.077\cdot 10^{1}$ & $1.027\cdot 10^{5}$ & $-9.872\cdot 10^{4}$\\
 &  &  & $2.203\cdot 10^{4}$ & $-1.613\cdot 10^{3}$ & $2.998\cdot 10^{1}$ & $-9.436\cdot 10^{4}$ & $9.754\cdot 10^{4}$ & $-2.223\cdot 10^{4}$ & $6.200\cdot 10^{2}$\\
 &  &  & $4.210\cdot 10^{1}$ & $-1.409\cdot 10^{5}$ & $1.079\cdot 10^{5}$ & $-3.457\cdot 10^{4}$ & $5.841\cdot 10^{3}$ & $-2.912\cdot 10^{2}$ & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $3.534\cdot 10^{-1}$ & $-5.574\cdot 10^{-1}$ & $1.072$ & $-3.666\cdot 10^{-3}$ & $7.260\cdot 10^{-5}$ & $-1.773\cdot 10^{-1}$ & $2.565\cdot 10^{-1}$\\
 &  &  & $-6.534\cdot 10^{-2}$ & $2.536\cdot 10^{-3}$ & $-4.109\cdot 10^{-5}$ & $-1.884$ & $1.251$ & $-3.110\cdot 10^{-1}$ & $2.203\cdot 10^{-2}$\\
 &  &  & $-4.862\cdot 10^{-4}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $-4.619\cdot 10^{-2}$ & $5.229\cdot 10^{-2}$ & $2.474\cdot 10^{-2}$ & $-1.276\cdot 10^{-3}$ & $2.427\cdot 10^{-5}$ & $1.326\cdot 10^{-1}$ & $-1.182\cdot 10^{-1}$\\
 &  &  & $3.585\cdot 10^{-2}$ & $-4.237\cdot 10^{-3}$ & $1.699\cdot 10^{-4}$ & $-1.195$ & $9.595\cdot 10^{-1}$ & $-2.689\cdot 10^{-1}$ & $2.794\cdot 10^{-2}$\\
 &  &  & $-7.915\cdot 10^{-4}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $-1.030\cdot 10^{2}$ & $1.461\cdot 10^{2}$ & $-6.233\cdot 10^{1}$ & $9.356$ & $-2.241\cdot 10^{-1}$ & $2.393\cdot 10^{2}$ & $-2.989\cdot 10^{2}$\\
 &  &  & $1.146\cdot 10^{2}$ & $-1.355\cdot 10^{1}$ & $3.712\cdot 10^{-1}$ & $4.241\cdot 10^{2}$ & $-4.257\cdot 10^{2}$ & $1.623\cdot 10^{2}$ & $-2.811\cdot 10^{1}$\\
 &  &  & $2.009$ & $3.352\cdot 10^{-2}$ & $6.497$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$r_1$} & \multirow{3}{*}{$h_3$} & $2.555\cdot 10^{-1}$ & $-1.456\cdot 10^{-1}$ & $1.182$ & $-1.057\cdot 10^{-2}$ & $2.431\cdot 10^{-4}$ & $1.614\cdot 10^{-1}$ & $-4.457\cdot 10^{-1}$\\
 &  &  & $-1.808\cdot 10^{-2}$ & $7.986\cdot 10^{-3}$ & $-1.921\cdot 10^{-5}$ & $-7.272$ & $5.457$ & $-7.552\cdot 10^{-1}$ & $3.301\cdot 10^{-2}$\\
 &  &  & $-1.667\cdot 10^{-3}$ & $6.677$ & $-4.969$ & $6.517\cdot 10^{-1}$ & $-6.629\cdot 10^{-2}$ & $4.739\cdot 10^{-3}$ & 
\\ \hline
\multirow{18}{*}{$f^{22}_{12}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_3$} & $-4.364\cdot 10^{4}$ & $9.766\cdot 10^{3}$ & $5.877\cdot 10^{3}$ & $-1.853\cdot 10^{3}$ & $-1.252\cdot 10^{1}$ & $4.023\cdot 10^{6}$ & $-3.048\cdot 10^{6}$\\
 &  &  & $8.156\cdot 10^{5}$ & $-9.070\cdot 10^{4}$ & $3.420\cdot 10^{3}$ & $-1.991\cdot 10^{7}$ & $1.563\cdot 10^{7}$ & $-4.337\cdot 10^{6}$ & $4.974\cdot 10^{5}$\\
 &  &  & $-1.902\cdot 10^{4}$ & $3.745\cdot 10^{7}$ & $-3.017\cdot 10^{7}$ & $8.634\cdot 10^{6}$ & $-1.029\cdot 10^{6}$ & $4.198\cdot 10^{4}$ & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $1.390$ & $-1.370$ & $1.264$ & $-2.252\cdot 10^{-2}$ & $6.813\cdot 10^{-4}$ & $-2.623$ & $2.207$\\
 &  &  & $-5.610\cdot 10^{-1}$ & $5.258\cdot 10^{-2}$ & $-1.710\cdot 10^{-3}$ & $-1.429\cdot 10^{-1}$ & $-2.820\cdot 10^{-1}$ & $1.256\cdot 10^{-1}$ & $-3.004\cdot 10^{-2}$\\
 &  &  & $1.735\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $-8.053\cdot 10^{-3}$ & $1.404\cdot 10^{-2}$ & $4.011\cdot 10^{-2}$ & $-2.327\cdot 10^{-3}$ & $3.380\cdot 10^{-5}$ & $7.970\cdot 10^{-2}$ & $3.213\cdot 10^{-3}$\\
 &  &  & $1.666\cdot 10^{-3}$ & $-4.446\cdot 10^{-4}$ & $6.597\cdot 10^{-5}$ & $-5.394\cdot 10^{-1}$ & $4.124\cdot 10^{-1}$ & $-1.209\cdot 10^{-1}$ & $1.210\cdot 10^{-2}$\\
 &  &  & $-3.351\cdot 10^{-4}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $-1.228\cdot 10^{3}$ & $8.470\cdot 10^{2}$ & $-1.994\cdot 10^{2}$ & $2.383\cdot 10^{1}$ & $-7.986\cdot 10^{-1}$ & $3.551\cdot 10^{3}$ & $-2.227\cdot 10^{3}$\\
 &  &  & $5.049\cdot 10^{2}$ & $-4.983\cdot 10^{1}$ & $1.891$ & $-3.867\cdot 10^{3}$ & $2.612\cdot 10^{3}$ & $-6.786\cdot 10^{2}$ & $8.736\cdot 10^{1}$\\
 &  &  & $-4.084$ & $3.253\cdot 10^{-7}$ & $2.033\cdot 10^{1}$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$r_1$} & \multirow{3}{*}{$h_3$} & $1.187$ & $-9.285\cdot 10^{-1}$ & $9.999\cdot 10^{-1}$ & $3.763\cdot 10^{-3}$ & $-2.319\cdot 10^{-4}$ & $-2.820\cdot 10^{1}$ & $1.856\cdot 10^{1}$\\
 &  &  & $-4.263$ & $4.173\cdot 10^{-1}$ & $-1.482\cdot 10^{-2}$ & $8.351\cdot 10^{1}$ & $-5.845\cdot 10^{1}$ & $1.462\cdot 10^{1}$ & $-1.588$\\
 &  &  & $6.166\cdot 10^{-2}$ & $-1.183\cdot 10^{2}$ & $9.199\cdot 10^{1}$ & $-2.595\cdot 10^{1}$ & $3.163$ & $-1.390\cdot 10^{-1}$ & \\
\cline{3-10} & \multirow{3}{*}{$r_2$} & \multirow{3}{*}{$h_3$} & $-9.328\cdot 10^{-2}$ & $-2.678\cdot 10^{-2}$ & $1.037$ & $9.548\cdot 10^{-4}$ & $-6.395\cdot 10^{-5}$ & $4.177$ & $-3.739$\\
 &  &  & $8.652\cdot 10^{-1}$ & $-8.863\cdot 10^{-2}$ & $2.853\cdot 10^{-3}$ & $-2.336\cdot 10^{1}$ & $1.746\cdot 10^{1}$ & $-4.658$ & $4.671\cdot 10^{-1}$\\
 &  &  & $-1.513\cdot 10^{-2}$ & $2.890\cdot 10^{1}$ & $-2.176\cdot 10^{1}$ & $5.886$ & $-6.174\cdot 10^{-1}$ & $2.042\cdot 10^{-2}$ & 
\\ \hline


==> fit_parameters_5.tex <==
\multicolumn{3}{c|}{}&$\uc_{-2,0}$&$\uc_{-1,0}$&$\uc_{0,0}$&$\uc_{1,0}$&$\uc_{2,0}$&$\uc_{-2,1}$&$\uc_{-1,1}$\\
\multicolumn{3}{c|}{}&$\uc_{0,1}$&$\uc_{1,1}$&$\uc_{2,1}$&$\uc_{-2,2}$&$\uc_{-1,2}$&$\uc_{0,2}$&$\uc_{1,2}$\\
\multicolumn{3}{c|}{}&$\uc_{2,2}$&$\uc_{-2,3}$ or $v$&$\uc_{-1,3}$ or $w$&$\uc_{0,3}$&$\uc_{1,3}$&$\uc_{2,3}$&\\
\hline
\multirow{18}{*}{$f^{22}_{21}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_3$} & $5.557\cdot 10^{4}$ & $-7.079\cdot 10^{4}$ & $1.715\cdot 10^{4}$ & $-1.715\cdot 10^{3}$ & $-1.776\cdot 10^{1}$ & $-2.156\cdot 10^{5}$ & $2.825\cdot 10^{5}$\\
 &  &  & $-4.954\cdot 10^{4}$ & $1.933\cdot 10^{3}$ & $1.669\cdot 10^{2}$ & $1.368\cdot 10^{6}$ & $-1.245\cdot 10^{6}$ & $2.867\cdot 10^{5}$ & $-2.528\cdot 10^{4}$\\
 &  &  & $7.764\cdot 10^{2}$ & $-4.187\cdot 10^{6}$ & $3.394\cdot 10^{6}$ & $-9.074\cdot 10^{5}$ & $9.857\cdot 10^{4}$ & $-3.665\cdot 10^{3}$ & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $1.882\cdot 10^{-1}$ & $-5.259\cdot 10^{-1}$ & $1.071$ & $-3.171\cdot 10^{-3}$ & $5.404\cdot 10^{-5}$ & $7.733\cdot 10^{-1}$ & $-2.626\cdot 10^{-1}$\\
 &  &  & $7.348\cdot 10^{-2}$ & $-1.274\cdot 10^{-2}$ & $5.236\cdot 10^{-4}$ & $-6.660$ & $4.802$ & $-1.270$ & $1.270\cdot 10^{-1}$\\
 &  &  & $-4.146\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $1.060\cdot 10^{-1}$ & $-5.702\cdot 10^{-2}$ & $4.575\cdot 10^{-2}$ & $-2.804\cdot 10^{-3}$ & $6.314\cdot 10^{-5}$ & $-6.956\cdot 10^{-1}$ & $3.783\cdot 10^{-1}$\\
 &  &  & $-4.457\cdot 10^{-2}$ & $2.390\cdot 10^{-4}$ & $1.079\cdot 10^{-4}$ & $-1.410$ & $1.272$ & $-3.958\cdot 10^{-1}$ & $4.609\cdot 10^{-2}$\\
 &  &  & $-1.596\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $-1.055\cdot 10^{1}$ & $5.062\cdot 10^{1}$ & $-3.404\cdot 10^{1}$ & $6.395$ & $-1.120\cdot 10^{-1}$ & $-6.162\cdot 10^{2}$ & $3.137\cdot 10^{2}$\\
 &  &  & $-1.303\cdot 10^{1}$ & $-6.257$ & $2.865\cdot 10^{-1}$ & $-2.943\cdot 10^{3}$ & $2.366\cdot 10^{3}$ & $-6.650\cdot 10^{2}$ & $8.050\cdot 10^{1}$\\
 &  &  & $-2.547$ & $2.233\cdot 10^{-5}$ & $1.410\cdot 10^{1}$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$r_1$} & \multirow{3}{*}{$h_3$} & $1.038$ & $-5.679\cdot 10^{-1}$ & $1.068$ & $-1.243\cdot 10^{-3}$ & $-2.006\cdot 10^{-5}$ & $2.342\cdot 10^{-1}$ & $-1.817$\\
 &  &  & $8.069\cdot 10^{-1}$ & $-9.209\cdot 10^{-2}$ & $3.094\cdot 10^{-3}$ & $-2.032\cdot 10^{1}$ & $1.695\cdot 10^{1}$ & $-5.364$ & $5.308\cdot 10^{-1}$\\
 &  &  & $-1.653\cdot 10^{-2}$ & $2.109\cdot 10^{1}$ & $-1.655\cdot 10^{1}$ & $4.900$ & $-4.785\cdot 10^{-1}$ & $1.384\cdot 10^{-2}$ & \\
\cline{3-10} & \multirow{3}{*}{$r_2$} & \multirow{3}{*}{$h_3$} & $7.914\cdot 10^{-1}$ & $-4.777\cdot 10^{-1}$ & $1.240$ & $-1.206\cdot 10^{-2}$ & $2.997\cdot 10^{-4}$ & $-1.221\cdot 10^{1}$ & $7.468$\\
 &  &  & $-1.483$ & $1.256\cdot 10^{-1}$ & $-3.795\cdot 10^{-3}$ & $3.867\cdot 10^{1}$ & $-2.554\cdot 10^{1}$ & $6.103$ & $-6.520\cdot 10^{-1}$\\
 &  &  & $2.428\cdot 10^{-2}$ & $-6.761\cdot 10^{1}$ & $5.032\cdot 10^{1}$ & $-1.388\cdot 10^{1}$ & $1.574$ & $-6.056\cdot 10^{-2}$ & 
\\ \hline
\multirow{15}{*}{$f^{22}_{22}$} & \multirow{3}{*}{$f_0$} & \multirow{3}{*}{$h_3$} & $3.181\cdot 10^{3}$ & $-2.943\cdot 10^{3}$ & $1.034\cdot 10^{3}$ & $-1.738\cdot 10^{2}$ & $3.794$ & $-4.607\cdot 10^{1}$ & $3.692\cdot 10^{3}$\\
 &  &  & $-2.022\cdot 10^{3}$ & $3.100\cdot 10^{2}$ & $-8.373$ & $-7.021\cdot 10^{3}$ & $-3.370\cdot 10^{3}$ & $3.125\cdot 10^{3}$ & $-4.570\cdot 10^{2}$\\
 &  &  & $1.735\cdot 10^{1}$ & $-6.421\cdot 10^{2}$ & $6.042\cdot 10^{3}$ & $-2.792\cdot 10^{3}$ & $2.879\cdot 10^{2}$ & $-7.221$ & \\
\cline{3-10} & \multirow{3}{*}{$\mu$} & \multirow{3}{*}{$h_2$} & $7.632\cdot 10^{-1}$ & $-8.366\cdot 10^{-1}$ & $1.128$ & $-7.494\cdot 10^{-3}$ & $1.431\cdot 10^{-4}$ & $-1.768$ & $1.144$\\
 &  &  & $-2.050\cdot 10^{-1}$ & $8.687\cdot 10^{-3}$ & $2.973\cdot 10^{-6}$ & $-2.322$ & $2.034$ & $-6.374\cdot 10^{-1}$ & $6.786\cdot 10^{-2}$\\
 &  &  & $-2.387\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\varsigma$} & \multirow{3}{*}{$h_2$} & $3.643\cdot 10^{-2}$ & $-3.122\cdot 10^{-3}$ & $3.526\cdot 10^{-2}$ & $-1.849\cdot 10^{-3}$ & $2.906\cdot 10^{-5}$ & $-2.354\cdot 10^{-1}$ & $8.167\cdot 10^{-2}$\\
 &  &  & $7.198\cdot 10^{-3}$ & $-3.667\cdot 10^{-3}$ & $2.186\cdot 10^{-4}$ & $-1.207$ & $1.091$ & $-3.367\cdot 10^{-1}$ & $3.876\cdot 10^{-2}$\\
 &  &  & $-1.290\cdot 10^{-3}$ &  &  &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$\lambda$} & \multirow{3}{*}{$h_{2,0}$} & $4.978\cdot 10^{2}$ & $-2.921\cdot 10^{2}$ & $1.700\cdot 10^{4}$ & $1.886$ & $-1.017\cdot 10^{-1}$ & $-2.462\cdot 10^{3}$ & $1.585\cdot 10^{3}$\\
 &  &  & $-6.078\cdot 10^{3}$ & $1.469\cdot 10^{1}$ & $-6.208\cdot 10^{-2}$ & $-9.783\cdot 10^{1}$ & $3.717\cdot 10^{2}$ & $6.634\cdot 10^{2}$ & $4.290\cdot 10^{1}$\\
 &  &  & $-1.855$ & $-1.696\cdot 10^{4}$ & $-3.431\cdot 10^{-1}$ &  &  &  & \\
\cline{3-10} & \multirow{3}{*}{$r_1$} & \multirow{3}{*}{$h_3$} & $-4.263\cdot 10^{-1}$ & $2.202\cdot 10^{-1}$ & $9.980\cdot 10^{-1}$ & $1.907\cdot 10^{-3}$ & $-5.164\cdot 10^{-5}$ & $1.817$ & $-1.112$\\
 &  &  & $2.470\cdot 10^{-1}$ & $-2.305\cdot 10^{-2}$ & $6.989\cdot 10^{-4}$ & $-8.017$ & $4.376$ & $-1.034$ & $9.458\cdot 10^{-2}$\\
 &  &  & $-3.066\cdot 10^{-3}$ & $8.023$ & $-4.755$ & $1.059$ & $-1.122\cdot 10^{-1}$ & $4.125\cdot 10^{-3}$ & 
\\ \hline

